Quantum Sensor Network Algorithms for Transmitter Localization

A quantum sensor (QS) is able to measure various physical phenomena with extreme sensitivity. QSs have been used in several applications such as atomic interferometers, but few applications of a quantum sensor network (QSN) have been proposed or developed. We look at a natural application of QSN -- localization of an event (in particular, of a wireless signal transmitter). In this paper, we develop effective quantum-based techniques for the localization of a transmitter using a QSN. Our approaches pose the localization problem as a well-studied quantum state discrimination (QSD) problem and address the challenges in its application to the localization problem. In particular, a quantum state discrimination solution can suffer from a high probability of error, especially when the number of states (i.e., the number of potential transmitter locations in our case) can be high. We address this challenge by developing a two-level localization approach, which localizes the transmitter at a coarser granularity in the first level, and then, in a finer granularity in the second level. We address the additional challenge of the impracticality of general measurements by developing new schemes that replace the QSD's measurement operator with a trained parameterized hybrid quantum-classical circuit. Our evaluation results using a custom-built simulator show that our best scheme is able to achieve meter-level (1-5m) localization accuracy; in the case of discrete locations, it achieves near-perfect (99-100\%) classification accuracy.

==> eaten.tex <==

para{Transmitter Localization using QSN.}
\blue{We propose to use quantum sensors that encode the transmitter's location information inside the sensors' quantum state and thus open up new opportunities for localization algorithms based on quantum properties.
We design two quantum algorithms that localize a transmitter using the quantum data received from a quantum sensor network.}
Our first quantum algorithm is based on \emph{quantum state discrimination} (QSD). 
It essentially involves posing the localization problem as a QSD problem~\cite{bergou-review-2007} which is to identify the specific state a given quantum state is in (from a given set of states in which the system can be) by performing quantum measurements on the given quantum system.
\blue{Solving a QSD problem is an established field~\cite{helstrom1969, Bae_2015} and we use pretty good measurement (PGM)~\cite{prettygood} to generate the measurement operators.}
The outcome of the measurement determines the quantum state, and thus, the location of the transmitter. 
However, the above process can be erroneous, as the state determined may be incorrect. 
So we develop a two-level (coarse level and fine level) approach that minimizes the probability of error while using QSD for localization.

\blue{Implementing POVM by PGM is non-trivial on current gate-based quantum computers~\cite{pra19-povm}, and it is especially difficult for a relatively large number of qubits~\cite{qcompiler}. 
Thus, we propose a more practical quantum algorithm based on trainable \emph{parameterized quantum circuits} (PQC)~\cite{Benedetti_2019}.
The measurement output of PQC is followed by some classical post-processing and a simple layer of neural network that determine the location of the transmitter.
The PQC-based approach circumvents the obstacle of implementing POVMs computed from PGM by ``training the POVM'' using some general PQCs.
Moreover, we observe that the localization performance of the PQC-based algorithm is better than the QSD-based algorithm.
We believe this is because the quantum circuits can learn the optimal parameters during the training processing on the quantum data collected from the quantum sensors.}
% In this context, the PQC-based method can be viewed as a trainable version of the QSD-based method.}
%%%%%

\blue{The overall architecture illustrated in Fig.~\ref{fig:quantumoverall} has two parts, the QSN part, and the quantum algorithm part.
In the QSN part, a probe state is generated and distributed to the quantum sensors.
Then, quantum sensors are impacted (the quantum state changed) due to the transmission from the transmitter's signal and the states will be teleported to a quantum computer through a quantum channel.
In the quantum algorithm part, either a QSD-based method or a PQC-based method is applied to predict the location of the transmitter.}
%\blue{To achieve this, all the sensor states need to be
%teleported to a centralized node for the global measurement.}
%%%%%%%%%%%%%%%%%%%
% Second, the quantum sensors make interactions with the signal sent from a transmitter. 
% The location of the transmitter is encoded in the quantum state at the quantum sensors.
% Third, the quantum states will be teleported~\cite{ton22-quantum} to a centralized node.
% Finally, at the central node, we consider global measurement where all the teleported qubits are measured simultaneously. 
% The measurement outcome indicates the location of the transmitter.
% Quantum measurement via positive operator-valued measure (POVM) is the core part of quantum state discrimination.
% POVM is the general quantum measurement defined as a set of positive semi-definite Hermitian matrices $\{E_i\}$ and each Hermitian matrix $E_i$ is associated with the measurement outcome $i$~\cite{qcqi-book}.
% In our context, we further associate an outcome $i$ to a two-dimensional location $(x, y)$.
% Thus, we discriminate the quantum state via POVM and the POVM's output indicates the transmitter location.






%For example, in the task of indoor RF localization, a transmitter signal's angle-of-arrival observed from different locations facilitates localization via triangulation~\cite{nsdi13-arraytrack}.

% \para{Potential of Quantum Sensors for Precise Localization.}
% Quantum sensing is an emerging field that leverages the quantum properties of light and matter at atomic/subatomic scales.
% The Laser Interferometer Gravitational-wave Observatory (LIGO) successfully detected \blue{weak gravitational wave signals from outer space caused by black-hole/neutron star merge. The use of squeezed state can further increase the sensitivity of the LIGO detector~\cite{ligo_2015}}.
% In~\cite{PRL20-qsn}, researchers use a reconfigurable distributed entangled RF-photonic quantum sensor network to estimate the amplitude and phase of a radio signal, and the estimation variance beats the standard quantum limit by over 3 dB~\cite{arizona21-thesis}.
% \blue{Advance in quantum technologies has led to the creation of efficient quantum radio-frequency (RF) sensors that are much more sensitive than traditional antenna-based RF sensors and are expected to cover the entire RF spectrum~\cite{PhysRevApplied.rydberg}.}
% \eat{They showed the performance of \blue{sensing a global property of the RF wave} is enhanced by leveraging a shared multipartite entangled state produced by squeezed light.}




% Quantum sensing is an emerging field that leverages the quantum properties of light and matter at atomic/subatomic scales.
% The Laser Interferometer Gravitational-wave Observatory (LIGO) successfully detected \blue{weak gravitational wave signals from outer space caused by black-hole/neutron star merge. The use of squeezed state can further increase the sensitivity of the LIGO detector~\cite{ligo_2015}}.
% In~\cite{PRL20-qsn}, researchers use a reconfigurable distributed entangled RF-photonic quantum sensor network to estimate the amplitude and phase of a radio signal, and the estimation variance beats the standard quantum limit by over 3 dB~\cite{arizona21-thesis}.
% \blue{Advance in quantum technologies has led to the creation of efficient quantum radio-frequency (RF) sensors that are much more sensitive than traditional antenna-based RF sensors and are expected to cover the entire RF spectrum~\cite{PhysRevApplied.rydberg}.}
% \eat{They showed the performance of \blue{sensing a global property of the RF wave} is enhanced by leveraging a shared multipartite entangled state produced by squeezed light.}
% %%%%%%%%%%%%%%%%
% \eat{\blue{In addition, a set of entangled $m$ sensors can further improve the precision factor by
% $1/\sqrt{m}$---known as reaching the Heisenberg limit.}}
% Motivated by the above, in this paper, we develop techniques for localization using a distributed
% quantum sensor network. 




% For the PQC-based methods, we use the TorchQuantum~\cite{hanruiwang2022quantumnas} library to implement and train the parameterized quantum circuits on a GPU.
% The localization process is similar to the QSD-based methods, except that the POVM is replaced by the PQC models described in Section~\ref{sec:pqc-loc}.



% , and the localization phase which repeats the process of the quantum sensor network generating then sending a quantum state and the localization schemes receiving then discriminating the quantum state.
% In particular, the localization schemes contain computing the probabilities for all possible measurement outcomes and sampling an outcome according to the probabilities.
% }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%We evaluate the discrete setting in terms of $\lacc$ only, and the continuous setting in terms
%of $\lerr$ only. 

% used for the discrete location setting, where we confine the location of the transmitters during both the training and localization phases to the center of the cells.
% $\lerr$ is used for the general continuous location setting, where the transmitters during the localization phase can be anywhere (the transmitters during the training phase are still at the cell center).
% Therefore, $\lacc$ is a percentage similar to the classification accuracy, and $\lerr$ is the distance between the ground truth location and the method's output location measured in meters.

\eat{When measuring the electric field strength in the real world, people measure the received power recorded by a spectrum analyzer, and the E-field is computed in the postprocessing by using the following formula~\cite{e-field-measure}
$$E = \sqrt{P \cdot (AF)^{2} \cdot Z}$$
where $P$ is the power in $watt$, $AF$ is the antenna factor, and $Z$ is the impedance ($50\ ohm$ by default).}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%We evaluate the discrete setting in terms of $\lacc$ only, and the continuous setting in terms
%of $\lerr$ only. 

% used for the discrete location setting, where we confine the location of the transmitters during both the training and localization phases to the center of the cells.
% $\lerr$ is used for the general continuous location setting, where the transmitters during the localization phase can be anywhere (the transmitters during the training phase are still at the cell center).
% Therefore, $\lacc$ is a percentage similar to the classification accuracy, and $\lerr$ is the distance between the ground truth location and the method's output location measured in meters.


% \blue{What should be the initial state?}
% Optimizing the POVM is governed by some metrics, such as the minimum error discrimination metric and the unambiguous discrimination metric~\cite{bergou2004}.
% Semi-definite programming~\cite{semidefinite} is a general numerical method that can compute the optimal POVM under various metrics.
% In our paper, we choose a simple but good enough method to compute a POVM, the pretty good measurement (PGM)~\cite{prettygood}


% We simulate $\hat{\rho_i}$ through our $\hat{U}(\alpha)$ model as if the transmitter is indeed at the location associated with $i$ and putting the initial probe state $\boldsymbol{\hat{\rho}_0}$ in a uniform superposition state.


% \para{Quantum State Discrimination.} 
% Our methodology is to pose the localization problem as a quantum state discrimination problem.
% Quantum state discrimination underlies various applications in quantum information processing tasks~\cite{bergou-review-2007}.
% It essentially describes the distinguishability of quantum systems in different states, and the general process of extracting classical information from quantum states~\cite{Bae_2015}.
% Fig.~\ref{fig:qsd} illustrates the process of quantum state discrimination, where one party (Alice) prepares a quantum state, and another party (Bob) measures the received quantum state sent by Alice.
% In our context of localization, the \emph{quantum sensor network plays the role of Alice}.
% And a \emph{central node that performs global measurement plays the role of Bob}.
% The problem of discriminating among non-orthogonal quantum states boils down to a measurement optimization problem, i.e., optimizing the POVM.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.32\textwidth]{figures/qsd.png}
%     \vspace{-0.1in}
%     \caption{Illustration of Quantum state discrimination. There are two parties: Alice for preparing and sending a quantum state, and Bob for measuring the received quantum state from Alice.}
%     \vspace{-0.1in}
%     \label{fig:qsd}
% \end{figure}

% \eat{\footnote{Our preliminary results show that an entangled initial probe state (instead of a simple uniform superposition state) will increase the localization performance. But this part is not included due to diluting this paper.}.}


% as a
% phase shift -- using an appropriate unitary operator. }
% We first formulate quantum sensing as a single parameter estimation problem, shown in Fig.~\ref{fig:unitary}.
% Consider a parameter $\alpha$ embedded in a unitary operator.
% To sense $\alpha$, one prepares an initial quantum state $\hat{\rho}_{0}$ and passes it through unitary operator $\hat{U}(\alpha)$, obtaining the output state:
% $\hat{\rho}(\alpha) = \hat{U}(\alpha) \hat{\rho}_{0} \hat{U}^{\dagger}(\alpha)$.
% $\hat{U}(\alpha)$ describes the interaction between a qubit and the environment~\cite{arizona21-thesis}


% Assume the initial state of the quantum sensor network is 
% $\ket{\boldsymbol{\psi_{0}}}$. 
% After the interaction with the environment, the quantum state evolves to $\ket{\boldsymbol{\psi_{\alpha}}} = \hat{U}(\boldsymbol{\alpha}) \ket{\boldsymbol{\psi_{0}}}$.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.26\textwidth]{figures/unitary.png}
%     \vspace{-0.1in}
%     \caption{Sensing modeled as a single parameter estimation problem. The initial state $\hat{\rho}_{0}$ is used to probe an unknown parameter $\alpha$ embedded in the unitary operator $\hat{U}(\alpha)$, yielding output state $\hat{\rho}(\alpha)$.}
%     \vspace{-0.1in}
%     \label{fig:unitary}
% \end{figure}



% If we can build a connection between the transmitter-receiver distance and some properties of the RF wave, we can model the $\hat{U}(\alpha)$ as a function of the RF wave.
% In this paper, we pick received signal strength (RSS) as the bridge that connects the $\alpha$ and the RF wave, because RSS is easily accessible and is widely used in the fingerprinting-based wireless localization field.
% We have
% \begin{equation}
%     \alpha = \frac{2\pi (RSS - NF)}{MP-NF}
%     \label{equ:alpha}
% \end{equation}
% \red{where $NF$ is the noise floor, $MP$ is the maximum power a sensor can receive.}
% We have $\alpha \in [0, 2\pi]$, since the received signal strength $RSS \in [NF, MP]$.
% Derived from Equation~\ref{equ:unitary_generator}, \ref{equ:generator}, \ref{equ:alpha}, the unitary operator at the sensor can be described as
% \begin{equation}
%     \hat{U}(\alpha)   = 
%     \begin{bmatrix}
%     e^{- i \frac{\pi (RSS - NF)}{MP-NF}} & 0\\
%     0 & e^{ i \frac{\pi (RSS - NF)}{MP-NF}}
%     \end{bmatrix}
%     \label{equ:unitary}
% \end{equation}


% For the RSS model, we use the log-distance model
% \begin{equation}
%     RSS(d) = P_0 - 10\beta log_{10}(d) + \mathcal{X}
%     \label{equ:propagation}
% \end{equation}
% where $P_0$ is the reference power a sensor receives at 1 meter away from the transmitter, $d$ is the transmitter-receiver distance, $\beta$ is the path-loss exponent, and $\mathcal{X}$ is the shadowing effect that can be represented by a zero-mean Gaussian distribution.


% To carry out sensing, one inputs $N$ probes in a quantum state $\hat{\boldsymbol{\rho_0}}$ and obtains the output quantum state,
% $\hat{\boldsymbol{\rho}}_N({\boldsymbol{\alpha}}) = \hat{U}(\boldsymbol{\alpha}) \hat{\boldsymbol{\rho}_0} \hat{U}^{\dagger}(\boldsymbol{\alpha})$,
% where the unknown parameters are $\boldsymbol{\alpha}=\{\alpha_n\}_{n=1}^{N}$, and each $\alpha_n$ represents an unknown parameter at the $n$th sensor. }

% \green{After modeling a single sensor, let us model multiple sensors in a distributed sensing scenario~\cite{Zhang_2021}.
% We assume $N$ unknown parameters at $N$ quantum sensors respectively. 
% The combined unitary operator is a \emph{tensor product} of $N$ individual unitary operators,
% $\hat{U}(\boldsymbol{\alpha}) = \bigotimes_{n=1}^{N} \hat{U}(\alpha_n)$.
% To carry out sensing, one inputs $N$ probes in a quantum state $\hat{\boldsymbol{\rho_0}}$ and obtains the output quantum state,
% $\hat{\boldsymbol{\rho}}_N({\boldsymbol{\alpha}}) = \hat{U}(\boldsymbol{\alpha}) \hat{\boldsymbol{\rho}_0} \hat{U}^{\dagger}(\boldsymbol{\alpha})$,
% where the unknown parameters are $\boldsymbol{\alpha}=\{\alpha_n\}_{n=1}^{N}$, and each $\alpha_n$ represents an unknown parameter at the $n$th sensor. }


% Take $\{ \rho_i \}$ with equal priors and compute the POVM $\{ E_i \}$ using PGM. 
%     During the training phase, if $\{ \rho_i \}$ are collected by a set of coarse-level sensors and the transmitter fingerprints at the center of the blocks, we get a coarse-level POVM $\{ cE_i \}$. }






%     A set of fine-level sensors collects quantum data $ \rho_i$ to determine the cell where the transmitter is in. 
     
   
% %%%%%%%%%%%%%
%     Likewise, if the  $\{ \rho_i \}$ are collected by a set of fine-level sensors and the transmitter fingerprints at the center of the cell of the associated block, we get fine-level POVM $\{ fE_i \}$.
%     Fig.~\ref{fig:povm-loc} (a) shows one coarse-level POVM and Fig.~\ref{fig:povm-loc} (b) shows four fine-level POVMs.
%     The dots in Fig.~\ref{fig:povm-loc} indicates the center of a block or cell.



% \begin{table}[h]
% \centering
% \caption{Runtime (s) for \povmone using 4 and 8 quantum sensors against varying grid size}
% \vspace{-0.1in}
% \begin{tabular}{||c | c | c|  c | c | c | c||} 
%  \hline
%   & 2x2 & 4x4 & 6x6 & 8x8 & 12x12 & 16x16\\
%  \hline
%  4 Sensors & 1.0 & 1.1 & 1.2 & 1.4 & 2.0 & 2.6\\ 
%  \hline
%  8 Sensors & 4.8 & 9.1 & 27.4 & 53.1 & 113.4 & 193.8\\ 
%  \hline
% \end{tabular}
% \vspace{-0.15in}
% \label{tab:runtime-onelevel}
% \end{table}

% \begin{table}[h]
% \centering
% \caption{Runtime (s) for three methods in $16\times 16$ grid}
% \vspace{-0.1in}
% \begin{tabular}{|| c | c | c ||} 
%  \hline
%  \povmone & \povm & \povmpro\\ 
%  \hline
%  193.8 & 10.3 & 11.3 \\ 
%  \hline
% \end{tabular}
% \vspace{-0.15in}
% \label{tab:runtime-compare}
% \end{table}





%%%%%%%%%  OLD Quantum Sensing Model  %%%%%%%%%%%%
% In our context, a quantum sensor evolves due to the received power over a time window. 
% Let the initial pure state of the sensor be $\ket{\psi_{0}}$, and let the impact on the sensor due to received power
% be represented by the unitary operator $U(\alpha)$ where $\alpha$ 
% depends on the received power, fixed time window over which the 
% sensor's state evolves, etc. The evolved state of the sensor
% is given by: $\ket{\psi_{\alpha}} = \hat{U}(\alpha) \ket{\psi_{0}}$.
% %%%%%%%%%%%%%%%%%%%%%%%%
% The unitary operator $\hat{U}(\alpha)$ describing the interaction between a 
% qubit and the environment is modeled as~\cite{ nature21_phase, arizona21-thesis, Zhang_2021}:
% \begin{equation}
%     \hat{U}(\alpha) = e^{-i\alpha \hat{G}}
%     \label{equ:unitary_generator}
% \end{equation}
% where $\hat{G}$ is the generator, which is a Hermitian operator.
% $\hat{G}$ depends on the type of $\alpha$ parameter~\cite{Zhang_2021} which includes 
% quadrature displacement~\cite{PRL20-qsn}, phase shift~\cite{nature21_phase}, 
% qubit phase rotation, etc.
% In our context, $\alpha$ is assumed to be a \emph{phase shift}, and thus, our generator follows the expression in~\cite{nature21_phase}: $\hat{G} = \sigma_z / 2$, where $\sigma_z$ is the Pauli-Z matrix.
% \eat{\begin{equation}
%     \hat{G} = \sigma_z / 2 = 
%     \begin{bmatrix}
%     \frac{1}{2} & 0\\
%     0 & -\frac{1}{2}
%     \end{bmatrix}
%     \label{equ:generator}
% \end{equation}}
% The phase shift $\alpha$ is fundamentally a function of the received power $P_R$, and we assume $\alpha$ to be directly proportional to $P_R$.
% \begin{equation}
%     \alpha = c P_R
%     \label{equ:alpha}
% \end{equation}
% where $c$ is an appropriate constant. From the above, we get 
% \begin{equation}
%     \hat{U}(\alpha)   = 
%     \begin{bmatrix}
%     e^{- i c P_R } & 0\\
%     0 & e^{ i c P_R}
%     \end{bmatrix}
%     \label{equ:unitary}
% \end{equation}
% Eqn.~\ref{equ:unitary} models how a quantum sensor evolves due to a received signal
% from a transmitter; in essence, the transmitter's signal triggers a phase shift in the quantum sensor. 

% Finally, we assume a simple signal propagation model, viz.,
% the log-distance model which gives $P_R$ (in dBm) as:
% \begin{equation}
%     P_0 - 10\beta \log_{10}(d) + \mathcal{X}    \label{equ:propagation}
% \end{equation}
% where $P_0$ is the transmit power (in particular, the power received at 1 m away from 
% the transmitter), $d$ is the Euclidean distance between the transmitter and the sensor, $\beta$ is the path-loss exponent, and $\mathcal{X}$ is the shadowing effect that can be represented by a zero-mean Gaussian distribution.
%%%%%%%%%  OLD Quantum Sensing Model  %%%%%%%%%%%%




% $$\hat{H}_V(t) = \hat{H}_{V_{{\parallel}}}(t) + \hat{H}_{V_{{\perp}}}(t)$$
% where $\hat{H}_{V_{\parallel}}$ is the parallel component of the Hamiltonian.
% $\hat{H}_{V_{\parallel}}$ leads to shifts of the energy levels of the sensor~\cite{RevModPhys.quantumsensing} and a corresponding change in the transition frequency ($\omega_0$ in Fig.~\ref{fig:quantumsensing}).
% $\hat{H}_{V_{\perp}}$ is the transverse component and it induces transitions between the two levels~\cite{RevModPhys.quantumsensing}, manifesting through an increased transition rate. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.16\textwidth]{figures/quantum-sensing.png}
%     \caption{A two-state quantum system.  $\ket{0}$ is the lower energy state and $\ket{1}$ is the higher energy state. Quantum sensing exploits changes in the energy level $E$ in response to an external signal $V(t)$.}
%     \vspace{-0.1in}
%     \label{fig:quantumsensing}
% \end{figure}

% \softpara{Assumption.}  The assumption is that the energy difference $\Delta E = E_1 - E_0$ is much larger than the energy changes in the Hamiltonian introduced by signal $V(t)$.

% This assumption is valid for most quantum sensing applications per~\cite{RevModPhys.quantumsensing}.
% Under this assumption, the transverse component  $\hat{H}_{V_{\perp}} (t)$ can be ignored~\cite{egerstrom}.
% Thus, 



the time evolution of the second period is reversed from negative to positive and the accumulated phase is nonzero
% $$\phi =  \int_{0}^{ \frac{T}{2}} \frac{\gamma}{\hbar} V_{\parallel}(t) dt - \int_{\frac{T}{2}}^{ T } \frac{\gamma}{\hbar} V_{\parallel}(t) dt = \frac{2}{\pi} \gamma E T \cos{\theta}$$ 
$ \phi = \int_{0}^{T} \frac{\gamma}{\hbar} V_{\parallel}(t) y(t) dt $,
where $y(t) = \pm1$ is the modulation function of the sequence that changes sign whenever a $\pi$ pulse is applied~\cite{PRL20-qsn}. So the phase shift $\phi_T$ within one cycle of sensing time $[0, T]$ is
$$ \phi_T = 2\times \int_{0}^{\sfrac{T}{2}} \frac{\gamma}{\hbar} V_{\parallel}(t) dt = \frac{2}{\pi \hbar} \gamma E T \cos{\theta} $$
If we assume $\theta=0$ or the $\pi$ pulse is applied whenever the $V_{\parallel}(t)$ changes sign (equivalent to square wave function), then
$ \phi_T = \frac{2}{\pi \hbar} \gamma E T$.
If the sensing time $t'=nT$, then the phase shift

==> saved-model.tex <==
\para{\red{Quantum Sensor Model}.} 
Impact on a quantum sensor due to a physical phenomenon is typically modeled by an appropriate unitary operator. 
Fig.~\ref{fig:quantumsensing} describes the basic features of a quantum sensor that has two levels of energy -- a sensor being represented as a qubit.
In general, the key quantity of quantum sensing is the quantum phase picked up by the sensor due to the interaction with the signal~\cite{RevModPhys.quantumsensing}. 
We want to use quantum sensors to detect presence/location of an RF transmitter, by measuring the quantum phase change that occurs during the sensing period.
In the following paragraphs, we derive the quantum phase change in an RF quantum sensor.

A quantum sensor's Hamiltonian $\hat{H}(t)$ can be broken into three components as~\cite{RevModPhys.quantumsensing}
$$\hat{H}(t) = \hat{H}_0 + \hat{H}_V(t) + \hat{H}_{control}(t)$$
where $\hat{H}(t)$ is the internal Hamiltonian of the system in the absence of an external signal. 
$\hat{H}_V(t)$ is the change in the Hamiltonian due to the external signal $V(t)$.
$\hat{H}_{control}(t)$ is the control Hamiltonian.
In a two-state system, $\ket{0}, \ket{1}$ are the eigenvectors of the sensor's internal Hamiltonian and hence correspond to energies $E_0, E_1$ respectively, see Fig.~\ref{fig:quantumsensing}.
The internal Hamiltonian $\hat{H}_0 = E_0 \ket{0}\bra{0} + E_1\ket{1}\bra{1}$.
The control Hamiltonian can be deliberately chosen so as to manipulate or tune the sensor in a controlled way~\cite{RevModPhys.quantumsensing}.
For simplicity, we can assume $\hat{H}_{control}=0$ in our analysis~\cite{egerstrom}.
Now let's focus on the signal Hamiltonian,
$$\hat{H}_V(t) = \hat{H}_{V_{{\parallel}}}(t) + \hat{H}_{V_{{\perp}}}(t)$$
where $\hat{H}_{V_{\parallel}}$ is the parallel component of the Hamiltonian.
$\hat{H}_{V_{\parallel}}$ leads to shifts of the energy levels of the sensor~\cite{RevModPhys.quantumsensing} and a corresponding change in the transition frequency ($\omega_0$ in Fig.~\ref{fig:quantumsensing}).
$\hat{H}_{V_{\perp}}$ is the transverse component and it induces transitions between the two levels~\cite{RevModPhys.quantumsensing}, manifesting through an increased transition rate. 

\begin{figure}
    \centering
    \includegraphics[width=0.16\textwidth]{figures/quantum-sensing.png}
    \caption{A two-state quantum system.  $\ket{0}$ is the lower energy state and $\ket{1}$ is the higher energy state. Quantum sensing exploits changes in the energy level $E$ in response to an external signal $V(t)$.}
    \vspace{-0.1in}
    \label{fig:quantumsensing}
\end{figure}

\softpara{Assumption.}  The assumption is that the energy difference $\Delta E = E_1 - E_0$ is much larger than the energy changes in the Hamiltonian introduced by signal $V(t)$.

This assumption is valid for most quantum sensing applications per~\cite{RevModPhys.quantumsensing}.
Under this assumption, the transverse component  $\hat{H}_{V_{\perp}} (t)$ can be ignored~\cite{egerstrom}.
Thus, 
$$\hat{H}_{V}(t) = \hat{H}_{V_{\parallel}}(t) = -\frac{1}{2}\gamma V_{\parallel}(t)\hat{\sigma}_z$$
where $\sigma_z$ is the Pauli-Z matrix, and $\gamma$ is the coupling of the qubit to the signal $V_{\parallel}(t)$.
So, the parallel component $\hat{H}_{V_{\parallel}}(t)$ induces a change in the spin in the $z$ axis direction, which is a qubit \emph{phase shift}.
${V_{\parallel}}(t)$ at the sensor is expressed as
$$V_{\parallel}(t) = E \sin(2\pi f  t + \theta)$$
where $E$ is the maximum electric field amplitude, $f$ is the frequency, and $\theta$ is the RF signal phase.
The unit of the coupling $\gamma$ is $J / (V\cdot m^{-1})$, and the unit of $V_{\parallel}(t)$ is $V\cdot m^{-1}$, the electric field strength.
It relates the changes in the quantum sensor's energy level to the external signal.
The coupling relationship between the quantum state and the signal is linear. 
$$\hat{H}(t) =  \hat{H}_0 + \hat{H}_{V_{\parallel}}(t) = 
\begin{pmatrix}
E_0 -\frac{1}{2}\gamma V_{\parallel}(t) & 0 \\
0 & E_1 + \frac{1}{2}\gamma V_{\parallel}(t)
\end{pmatrix}$$
Assume at time $t=0$, the quantum state is $\ket{\phi_0}$. Then at time $t=t'$, the state $\ket{\phi_{t'}}$ is,
$$ \ket{\psi_{t'}} = \hat{U}(0, t') \ket{\psi_0} $$
where the time evolution operator $\hat{U}(0, t') = e^{\frac{i}{\hbar} \int_{0}^{t'} \hat{H}(t) dt} $ is,
$$\hat{U}(0, t') =
\begin{pmatrix}
e^{\frac{i}{\hbar}(E_0 t' - \int_{0}^{t'} \frac{1}{2}\gamma V_{\parallel}(t) dt)} & 0 \\
0 & e^{\frac{i}{\hbar}(E_1 t' + \int_{0}^{t'} \frac{1}{2}\gamma V_{\parallel}(t) dt)}
\end{pmatrix}$$
where $\hbar=6.626\times 10^{-34} J\cdot s$ is the plank constant.
$E_0, E_1$ are known constants since we construct the system.
We fix the time $t'$ for which the system is allowed to evolve under the external signal.
We observe that the phase shift comes from two parts. 
The first part $\frac{\Delta E t'}{\hbar}$ is a constant since $\Delta E = E_1 - E_0$ and $t'$ are both constants.
The second part $\int_{0}^{t'} \frac{\gamma}{\hbar} V_{\parallel}(t) dt$ is a function of the signal received at the quantum sensor that encodes the location information of the transmitter.

Let's take an analysis of the phase shift accumulated during the sensing time $t \in [0, t']$ due to the signal $V(t)$.
We assume $t' = T = \sfrac{1}{f}$, exactly one cycle. 
The phase shift in one cycle
$$\phi =  \int_{0}^{T} \frac{\gamma}{\hbar} V_{\parallel}(t) dt$$ due to the signal is zero because the positive phase buildup during the first half of $T$ is exactly canceled by the negative phase buildup during the second half of $T$.
To compensate for this, We invert the qubit at time $T/2$ using a $\pi$ pulse~\cite{RevModPhys.quantumsensing}, the time evolution of the second period is reversed from negative to positive and the accumulated phase is nonzero
% $$\phi =  \int_{0}^{ \frac{T}{2}} \frac{\gamma}{\hbar} V_{\parallel}(t) dt - \int_{\frac{T}{2}}^{ T } \frac{\gamma}{\hbar} V_{\parallel}(t) dt = \frac{2}{\pi} \gamma E T \cos{\theta}$$ 
$ \phi = \int_{0}^{T} \frac{\gamma}{\hbar} V_{\parallel}(t) y(t) dt $,
where $y(t) = \pm1$ is the modulation function of the sequence that changes sign whenever a $\pi$ pulse is applied~\cite{PRL20-qsn}. So the phase shift $\phi_T$ within one cycle of sensing time $[0, T]$ is
$$ \phi_T = 2\times \int_{0}^{\sfrac{T}{2}} \frac{\gamma}{\hbar} V_{\parallel}(t) dt = \frac{2}{\pi \hbar} \gamma E T \cos{\theta} $$
If we assume $\theta=0$ or the $\pi$ pulse is applied whenever the $V_{\parallel}(t)$ changes sign (equivalent to square wave function), then
$ \phi_T = \frac{2}{\pi \hbar} \gamma E T$.
If the sensing time $t'=nT$, then the phase shift 
$$\phi = n\phi_T =  \frac{2n}{\pi \hbar} \gamma E T$$
% Recall the assumption that $\Delta E$ is much larger than the energy changes brought by the signal Hamiltonian.
% So if $n\phi_T$ is some value within $2\pi$, then the constant $\frac{\Delta E t'}{\hbar}$ will be a large value that is a lot bigger than $2\pi$.
Since the sensing time is fixed, the phase shift caused by the internal Hamiltonian can be viewed as a constant. 
But the phase shift caused by the signal Hamiltonian is not a constant and is affected by the external signal.
The larger the electric field $E$ is at the sensor, the larger the phase shift will incur by the signal.
The electric field strength can be modeled as a function of the distance between the transmitter and the sensor.
That is, the larger the distance a sensor is to a transmitter, the smaller the electric field the sensor receives from the transmitter.
This key relationship will be utilized to localize the transmitter.
\blue{The details of the electric field model are presented in the evaluation section.}

% From all the above, we have
% $$ \ket{\psi(t_1)} = \hat{U}(t_0, t_1) \ket{\psi(t_0)} = e^{ -\frac{1}{2} i \hat{\sigma}_z \int_{t_0}^{t_1} \frac{\gamma}{\hbar} V_{\parallel}(t) y(t) dt } \ket{\psi(t_0)} $$
% where $\ket{\psi(t_0)}$ is the initial state, and $\ket{\psi(t_1)}$ is the state after the interaction with the signal after a sensing period.
% Assuming $t_1 - t_0 = nT$, the evolved state at time $t_1$ is
